Ensuring Ground Truth Accuracy in Healthcare with the EVINCE framework

Misdiagnosis is a significant issue in healthcare, leading to harmful consequences for patients. The propagation of mislabeled data through machine learning models into clinical practice is unacceptable. This paper proposes EVINCE, a system designed to 1) improve diagnosis accuracy and 2) rectify misdiagnoses and minimize training data errors. EVINCE stands for Entropy Variation through Information Duality with Equal Competence, leveraging this novel theory to optimize the diagnostic process using multiple Large Language Models (LLMs) in a structured debate framework. Our empirical study verifies EVINCE to be effective in achieving its design goals.

==> ConfusionMatrices.tex <==
\section{Confusion Matrices}

Our empirical study shows that 
when the three LLMs independently perform
disease prediction based on their own knowledge,
without any supplemental data such as RAG or 
context, GPT-4 outperforms Gemini by
about 2.5\% and Claude $5\%$.  When SocraSynth
is employed to orchestrate debates between a pair
of LLMs, the prediction accuracy improves to $83.5\%$
with negligible statistical significance.  

After performing a deep dive into 
the results, there exhibit two interesting patterns.
First, though Gemini and Claude trail GPT-4 
by a few percentile in prediction accuracy, once 
a debate has been administrated, both Gemini-GPT4
and Claude-GPT4 make up to five percentile
improvement.  Examining the results in details,
the three LLMs perform well in similar categories
such as {}, but they make mistakes in different 
diseases.  Liver diseases, heart diseases, and skin
infections are three categories that confuse
all LLMs.




without debate, GPT-4
performs markedly better over Gemini by about
$2.5\%$ and over Claude by $5\%$. 
However, when 

